Denoising Diffusion Probabilistic Models for Magnetic Resonance Fingerprinting

Magnetic Resonance Fingerprinting (MRF) is a time-efficient approach to quantitative MRI, enabling the mapping of multiple tissue properties from a single, accelerated scan. However, achieving accurate reconstructions remains challenging, particularly in highly accelerated and undersampled acquisitions, which are crucial for reducing scan times. While deep learning techniques have advanced image reconstruction, the recent introduction of diffusion models offers new possibilities for imaging tasks, though their application in the medical field is still emerging. Notably, diffusion models have not yet been explored for the MRF problem. In this work, we propose for the first time a conditional diffusion probabilistic model for MRF image reconstruction. Qualitative and quantitative comparisons on in-vivo brain scan data demonstrate that the proposed approach can outperform established deep learning and compressed sensing algorithms for MRF reconstruction. Extensive ablation studies also explore strategies to improve computational efficiency of our approach.

==> sections/header_tmi.tex <==
%\author{First A. Author, \IEEEmembership{Fellow, IEEE}, Second B. Author,and Third C. Author, Jr., \IEEEmembership{Member, IEEE}
\author{Perla Mayo, Carolin M Pirkl, Alin Achim, Bjoern H Menze and Mohammad Golbabaee 
\thanks{%Firstly submitted on October, 2024. 
PM, AA and MG are with the University of Bristol, UK. CMP is with GE HealthCare, Munich, Germany. BHM is with the University of Zurich, Switzerland. PM and MG are the corresponding authors (e-mail: pm15334@bristol.ac.uk and m.golbabaee@bristol.ac.uk, respectively).}
}


\maketitle
%
\begin{abstract}
%\redparen{Abstract needs re-write}
Magnetic Resonance Fingerprinting (MRF) is a time-efficient approach to quantitative MRI, enabling the mapping of multiple tissue properties from a single, accelerated scan. However, achieving accurate reconstructions remains challenging, particularly in highly accelerated and undersampled acquisitions, which are crucial for reducing scan times. While deep learning techniques have advanced image reconstruction, the recent introduction of diffusion models offers new possibilities for imaging tasks, though their application in the medical field is still emerging. Notably, diffusion models have not yet been explored for the MRF problem. In this work, we propose for the first time a conditional diffusion probabilistic model for MRF image reconstruction. Qualitative and quantitative comparisons on in-vivo brain scan data demonstrate that the proposed approach can outperform established deep learning and classical compressed sensing algorithms for MRF reconstruction. A range of ablation studies also explore strategies to improve computational efficiency of our approach.

\end{abstract}

\begin{IEEEkeywords}
Denoising diffusion probabilistic models, quantitative magnetic resonance imaging, magnetic resonance fingerprinting, image reconstruction.
\end{IEEEkeywords}


==> sections/intro.tex <==
% ==============================================================
% = I N T R O D U C T I O N
% ==============================================================
\section{Introduction}
\label{sec:intro}
Quantifying the intrinsic nuclear magnetic resonance (NMR) properties of tissues~\cite{tofts2005quantitative} provides a powerful tool for tissue characterization and monitoring of pathological changes. However, conventional quantitative MRI (qMRI) techniques face challenges due to long acquisition times, limiting their clinical utility. This is because qMRI often requires sampling a long  sequence (time series) of magnetization images to capture tissue properties, making it difficult to acquire the full spatiotemporal volume in a reasonable scan time. Magnetic Resonance Fingerprinting (MRF)~\cite{ma2013mrf} and other transient-state imaging techniques~\cite{jiang2015fisp,gomez2019qtimrf,cao2022tgas} were introduced to address this problem. To reduce scan time, MRF uses short-length acquisition sequences to encode multiple tissue properties simultaneously and applies compressed sensing to subsample only a fraction of the spatio-temporal k-space data. However, faster scans lead to challenges in image reconstruction, including aliasing artifacts from k-space undersampling and limited tissue property information due to the truncated acquisition sequences. Effective image reconstruction algorithms are needed to tackle these challenges and improve the accuracy and precision of tissue parameter estimation.

Early MRF imaging algorithms~\cite{ma2013mrf,mcgivney2014svdmrf} used gridding reconstruction (non-Cartesian Fourier back-projection) to convert undersampled k-space data into image time series. Tissue properties were then estimated through dictionary matching, where voxel time signals were compared to a precomputed dictionary of theoretical tissue fingerprints. However, the accuracy of these methods was limited by aliasing artifacts that were not addressed during the image reconstruction step. While later compressed sensing algorithms~\cite{mazor2018flor,zhao2018lowrank,hamilton2019simultaneous,lima2019sparsity,hu2021highqualitymrf} introduced various sparsity and/or low-rank priors to regularize reconstruction and reduce artifacts, the most effective MRF algorithms to date are data driven, based on deep learning~\cite{balsiger2018mrf,fang2019supervisedmrf,golbabaee2019geometry,soyak2021convica,fatania2022plug,hamilton2022dipmrf,li2023learnedtensor}. These methods use some form of convolutional neural networks (CNNs) to directly learn spatio-temporal priors from the data, allowing them to more accurately restore (de-alias) MRF image time series or reconstruct quantitative maps.

Recently, denoising diffusion probabilistic models (DDPM) \cite{dpm2015,ho2020ddpm,nichol2021iddpm,song2021ddim} have gained significant attention due to their remarkable performance on image generation~\cite{dhariwal2021ddpmbeatgans,rombach2022hrimagesynth,hoogeboom2023simplediffusion} and image restoration tasks~\cite{choi2021ilvr,xie2023smartbrush,saharia2022imagesriterative,ozdenizci2023patchddpm,xia2023diffir}. Built on a hierarchy of denoising autoencoders, DDPMs are trained to iteratively refine image details by denoising and reversing a diffusion process. While their applications in medical imaging are emerging (e.g. in segmentation~\cite{wu2024medsegdiff,wolleb2022diffusionmedseg}, image-to-image translation~\cite{ozbey2023adversarialdiffusion,li2023zeroshottranslation}, and image reconstruction~\cite{liu2023dolce,xu2023zeroshotct,peng2022towardsmrdiffusion}), their potential for MRF imaging is yet unexplored. Compared to CNNs, the current state-of-the-art for MRF reconstruction, DDPMs offer several advantages. DDPMs' iterative refinement allows for stage-wise, progressive restoration of image details from coarse to fine scales, leading to more precise recovery compared to the single-pass structure of CNNs. They also incorporate advanced mechanisms like self-attention~\cite{vaswani2017attention} or transformers~\cite{dosovitskiy2020transformers}, which more effectively model long-range pixel dependencies. Additionally, while CNNs treat image restoration as a deterministic mapping from a corrupted to a restored image, DDPMs operate within a probabilistic framework, allowing them to learn the distribution of possible solutions for a given task and generate multiple samples i.e. a useful feature for capturing uncertainties in the reconstructed images. 

This paper presents, to the best of our knowledge, the first diffusion-based model for MRF image reconstruction. We train a conditional DDPM model to generate restored MRF image time series from initial gridding reconstructions, which suffer from aliasing artifacts due to accelerated MRF acquisitions. Evaluated on in-vivo brain scans data, we show that the proposed approach outperforms established deep learning and standard compressed sensing MRF algorithms in terms of image reconstruction and quantitative mapping accuracies. Additionally, the probabilistic nature of DDPM allows us to generate multiple sample reconstructions given an input and produce a variance map to visualize reconstruction uncertainties. To address the computational challenges associated with training diffusion models on high-dimensional MRF data, we employed a subspace dimensionality reduction approach from~\cite{mcgivney2014svdmrf} to temporally compress the MRF image time series, enabling the diffusion process to operate within a reduced latent space. We further implemented a patch-based processing pipeline to efficiently handle the spatial dimensions of data, enabling training and reconstruction on modest GPUs with limited memory and reasonable runtimes. 
